To ChatGPT, or not to ChatGPT: That is the question!

ChatGPT has become a global sensation. As ChatGPT and other Large Language Models (LLMs) emerge, concerns of misusing them in various ways increase, such as disseminating fake news, plagiarism, manipulating public opinion, cheating, and fraud. Hence, distinguishing AI-generated from human-generated becomes increasingly essential. Researchers have proposed various detection methodologies, ranging from basic binary classifiers to more complex deep-learning models. Some detection techniques rely on statistical characteristics or syntactic patterns, while others incorporate semantic or contextual information to improve accuracy. The primary objective of this study is to provide a comprehensive and contemporary assessment of the most recent techniques in ChatGPT detection. Additionally, we evaluated other AI-generated text detection tools that do not specifically claim to detect ChatGPT-generated content to assess their performance in detecting ChatGPT-generated content. For our evaluation, we have curated a benchmark dataset consisting of prompts from ChatGPT and humans, including diverse questions from medical, open Q&A, and finance domains and user-generated responses from popular social networking platforms. The dataset serves as a reference to assess the performance of various techniques in detecting ChatGPT-generated content. Our evaluation results demonstrate that none of the existing methods can effectively detect ChatGPT-generated content.

==> table/analysis.tex <==
\renewcommand\tabularxcolumn[1]{m{#1}}
\begin{tabularx}{\textwidth}{|l|X|c|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{Approach}} & \multicolumn{1}{c|}{\textbf{Limitations}}   & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Tool \\ Availability\end{tabular}}} & \textbf{TPR(\%)} & \textbf{TNR(\%)} \\ \hline

Draft and Goal~\cite{DAG} &  The tool over-classify text as being human-written          & \checkmark                    & 1.7 & 98.7                                  \\ \hline

Writefull GPT Detector~\cite{writefull} &  The tool consistently classified AI-generated texts with a probability score of no higher than ~40\%          & \checkmark                    & 1.8         & 98.6                         \\ \hline

Writer AI Content Detector~\cite{WriterAIContentDetector} & 
An AI content detector that works for \textit{GPT-3}, \textit{GPT-4}, and \textit{ChatGPT}.
%The tool over-classify text as being human-written          
& \checkmark                    & 1.4         & 98.8                         \\ \hline

Content at Scale~\cite{aicontentdetector}  & 
An online tool that works for \textit{ChatGPT}.
It assigns excessive weight to the predictability feature while determining whether a text is AI-generated.
& \checkmark                    & 28.5     & 85.7                             \\ \hline

Hugging Face~\cite{Huggingface}  & 
A tool released by Hugging Face for detecting text generated from \textit{ChatGPT}.
The tool tends to over-classify text as being human-written          
& \checkmark                    & 9.1    & 96.9                              \\ \hline

Cotton et al. \cite{cotton2023ensuring}   & ChatGPT is prone to claim that the text was generated by it, even when this is not true       & \checkmark       & 27.1 & 64.8                                                \\ \hline

Kumarage et al. \cite{kumarage2023stylometric}  & 
Sequence-based detection %require human and AI-generated text
using stylometric signals to detect AI-generated tweets.
%. The tool tends to \mbox{over-classify} text as being human-written                                   
& \checkmark           & 13.3 & 84.7                                  \\ \hline

Copyleaks~\cite{copyleaks} & The tool over-classify text as being human-written          & \checkmark                    & 1.5    & 98.7                              \\ \hline

Ma et al. \cite{ma2023abstract} & It is difficult to automatically detect factual inconsistencies in the generated text                & -                    & -     & -                              \\ \hline

Khalil et al. \cite{khalil2023will}& The authors conducted only the analysis. Not an actual tool was designed. Focused only on the academic field    & -    & -      & -                              \\ \hline

Corrector App~\cite{correctorapp} & The tool over-classify text as being human-written          & \checkmark                    & 7.4  & 98.8                                \\ \hline

Mitrović et al. \cite{mitrovic2023chatgpt}  & Only studied the pros and cons of plagiarism effect of ChatGPT in the academic field                                                    & -                    & -             & -                  \\ \hline 

Mitchell et al. \cite{mitchell2023detectgpt}  & 
Specifically developed to detect  text generated by \textit{GPT-2}
The tool works only with 48 tokens or more 
& \checkmark         & 14.9          & 96.4                       \\ \hline

GPTZero~\cite{GPTZero} & 
A classification model that determines whether a document was written by an LLM, providing predictions on a sentence, paragraph, and document level.
It mainly works for content in the English language. 
The tool tends to over-classify text as being human-written          
& \checkmark                    & 8.3     & 95.1                             \\ \hline

Guo et al. \cite{guo2023close} & 
Created for \textit{ChatGPT}, this tool underwent comprehensive human evaluations and linguistic analyses of \textit{ChatGPT}-generated content compared with that of humans.
The proposed available dataset is highly unbalanced and comprises anomalous text instances.
& \checkmark                    & 44.6 & 98.6                          \\ \hline

Bleumink et al. \cite{bleumink2023keeping} & 
A web-based AI detection tool to determine or detect whether a human or ChatGPT generated the text given. 
Performed experiments only on educational data. 
Does not specify the patterns found in the dataset analysis                           
& \checkmark         & 21.8              & 92.5                  \\ \hline

OpenAI Text Classifier~\cite{AITextClassifier} & 
A fine-tuned \textit{GPT} model that predicts the likelihood that a piece of text is AI-generated from a variety of sources, including \textit{ChatGPT}.
The tool works only with 1000 characters or more and is less prone to be sure that a  text was artificially generated.
& \checkmark                    & 17.9  & 85.7                                 \\ \hline

ZeroGPT~\cite{AITextDetector} & 
Specifically developed to detect OpenAI text.
Limited capabilities with shorter text.           
& \checkmark                    & 32.5         &   92.3                       \\ \hline

Gao et al. \cite{gao2022comparing}  & Very focused on academic abstracts. Using the existing detection tools for analysis                                                     & -                     & -                      & -                  \\ \hline

Kushnareva et al. \cite{kushnareva2021artificial}  & 
Need white box access to the attention maps of the model generating text, the available code uses \textit{BERT} attention maps.
It performs \textit{Topological Data Analysis} on the data for AI-generated text detection. 
The authors state that it is robust against unseen prompts from GPT models.
& \checkmark              & 24.1   & 89.3                               \\ \hline

Fröhling et al. \cite{Frohling2021feature} & 
The algorithm uses feature-based detection to identify automated language models such as GPT-2, GPT-3, and Grover.
The detection  becomes less accurate with increasing text complexity.        
& \checkmark                     & 23.8 & 89.2                                \\ \hline

Zellers et al. \cite{zellers2019defending} & 
State-of-the-Art Defense against Neural Fake News. 
The only focus is fake news, no research on GPT models was conducted.
Do not consider adversarial robustness~\cite{Frohling2021feature}.                                                                      
& \checkmark         & 23.1 & 91.3
                                     \\ \hline

Solaiman et al. \cite{solaiman2019release} & 
Specifically developed to detect  text generated by \textit{GPT-2}
& \checkmark         & 7.4 & 97.8                                     \\ \hline

Gehrmann et al. \cite{gehrmann2019gltr} & 
It utilizes the distributional properties of the underlying text used for the model. 
It was tested on the prompts from GPT-2 1.5B parameter model.
Allows only visual classification, making it a human manual detection. 
The tool needs tuning and customization for each specific task. 
& \checkmark         & 21.7 & 94.2                          \\ \hline

Nguyen-Son et al. \cite{nguyen2017identifying}  & The effectiveness varies with input text length. Tested only on text produced by a particular version of Google Translate     & -             & -     & -                   \\ \hline

Aharoni et al. \cite{aharoni2014automatic}  & Main focus is only on text translation     & -                    & -  & -                                    \\ \hline
\end{tabularx}

==> table/analysis_functionality.tex <==
\renewcommand\tabularxcolumn[1]{m{#1}}
\begin{tabularx}{\textwidth}{|l|X|X|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{Approach}}    & \multicolumn{1}{c}{\textbf{Functionality}}                                                                                              & \multicolumn{1}{c|}{\textbf{Limitations}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Tool \\ Availablity\end{tabular}}} & \textbf{TPR} \\ \hline

Draft and Goal~\cite{DAG} & Analyzes different fingerprints left by the AI models to determine if a text was Ai-generated & The tool over-classify text as being human-written          & \checkmark                    & 1.7                                  \\ \hline


Copyleaks~\cite{copyleaks} & $No Information Available$   & The tool over-classify text as being human-written          & \checkmark                    & 1.5                                  \\ \hline

Writefull GPT Detector~\cite{writefull} & $No Information Available$   & The tool consistently classified AI-generated texts with a probability score of no higher than ~40\%          & \checkmark                    & 1.8                                  \\ \hline

Corrector App~\cite{correctorapp} & AI-generated text detection using proprietary GPT-3 algorithm   & The tool over-classify text as being human-written          & \checkmark                    & 0.9                                  \\ \hline

Writer AI Content Detector~\cite{WriterAIContentDetector} & $No Information Available$    & The tool over-classify text as being human-written          & \checkmark                    & 1.4                                  \\ \hline

Content at Scale~\cite{aicontentdetector} & AI-generated text detection and creation    & It assigns excessive weight to the predictability feature while determining whether a text is an AI-generated          & \checkmark                    & 28.5                                  \\ \hline

Hugging Face~\cite{Huggingface}  & $No Information Available$  & The tool tends to over-classify text as being human-written          & \checkmark                    & 9.1                                  \\ \hline

Cotton et al. \cite{cotton2023ensuring} & AI-generated text detection using ChatGPT itself  & ChatGPT is prone to claim that the text was generated by it, even when this is not true              & -                    & -                                  \\ \hline

Kumarage et al. \cite{kumarage2023stylometric} & Stylometric Detection of AI-generated text & Sequence-based detection, require both human and AI-generated text                                   & \checkmark           & -                                  \\ \hline

Ma et al. \cite{ma2023abstract} & AI-generated text detection based on the "writing style"  & It is difficult to automatically detect factual inconsistencies in the generated text                & -                    & -                                   \\ \hline

Khalil et al. \cite{khalil2023will} & Evaluation of plagiarism detectors on AI-generated essays  & The authors conducted only the analysis. Not an actual tool was designed. Focused only on the academic field    & -    & -                                    \\ \hline

Mitrović et al. \cite{mitrovic2023chatgpt} & AI-generated text detection based on fine-tuned DistilBERT                                                     & Only studied the pros and cons of plagiarism effect of ChatGPT in the academic field                                                    & -                    & -                               \\ \hline 

Mitchell et al. \cite{mitchell2023detectgpt} & AI-generated text detection using log probabilities computed by a generative model                             & Limited in the number of token that it can analyze                                                                                      & \checkmark         & -                                 \\ \hline

GPTZero~\cite{GPTZero} & AI-generated text, with a focus on English prose  & The tool tends to over-classify text as being human-written          & \checkmark                    & 8.3                                  \\ \hline

Guo et al. \cite{guo2023close} & Analysis of the linguistic and the stylist characteristic of the ChatGPT and human feedback to detect patterns & Limited in the detection capability. The dataset is highly unbalanced and comprises anomalous text instances                                                                   & \checkmark                    & \checkmark                          \\ \hline

Bleumink et al. \cite{bleumink2023keeping} & Designed a web-based detection tool to detect texts in the education field                                     & Performed experiments only on the education data. Does not specify the patterns found in the dataset analysis                           & \checkmark         & -                                \\ \hline

OpenAI Text Classifier~\cite{AITextClassifier} & ChatGPT text detection using a fine-tuned GPT model  & Similar to Cotton et al. \cite{cotton2023ensuring} the capabilities of the tool are limited for the same reasons            & \checkmark                    & 27.9                                  \\ \hline

GPTZero~\cite{GPTZero} & AI-generated text detection using DeepAnalyse\texttrademark Technology & $No Information Available$             & \checkmark                    & 32.5                                  \\ \hline

Gao et al. \cite{gao2022comparing} & Evaluation of plagiarism detectors on AI-generated abstract                                                    & Very focused on academic abstracts. Using the existing detection tools for analysis                                                     & -                     & -                                        \\ \hline

Kushnareva et al. \cite{kushnareva2021artificial} & Topological Data Analysis for AI-generated text detection                                                      & Need white box access to the attention maps of the model generating text                                                                & \checkmark              & -                                  \\ \hline

Fröhling et al. \cite{Frohling2021feature} & Feature classifier for AI-generated text detection                                                             & The detection  becomes more difficult with increasing model complexity                                                                  & \checkmark                     & \checkmark                                \\ \hline

Zellers et al. \cite{zellers2019defending} & Fake news creation and detection                                                                               & Do not consider adversarial robustness. The only focus is fake news                                                                     & \checkmark         & -                                     \\ \hline

Solaiman et al. \cite{solaiman2019release} & Analysis of the human detection, automated ML-based detection of synthetic texts using 3 models                & Limited in the detection capability. Able to detect only the text generated by ChatGPT-2                                                & \checkmark         & -                                      \\ \hline

Gehrmann et al. \cite{gehrmann2019gltr} & Support tool for manual AI-generated text detection                                                            & The detection is only visual, and the detection has to be made manually. The tool needs tuning and customization for each specific task & \checkmark         & -                         \\ \hline

Nguyen-Son et al. \cite{nguyen2017identifying} & Detection of AI-generated text using statistical  analysis  & The effectiveness varies with the length of text in input. Tested only on text produced by a particular version of Google Translate     & -             & -                        \\ \hline

Aharoni et al. \cite{aharoni2014automatic} & Detection of AI-translated text using automatic text classification methods with common content-independent linguistic features  & Main focus is only on text translation     & -                    & -                                      \\ \hline
\end{tabularx}

==> table/comparison_survey.tex <==
\begin{tabular}{ccccc}
\textbf{Author(s)} & \textbf{Design, aims}                                                                         & \textbf{Limitations}                                                                                                                                                                                                                       & \textbf{Available} & \textbf{Tested on GPT-3} \\ \hline
Solaiman et al.                     & Analysis of the human detection and automated ML-based detection of synthetic texts using 3 models             & Limited in the detection capability. Also, it detects only the text generated by ChatGPT-2                                                                                                                                                                  & Online Tool                         & No                                        \\ \hline
Guo et al.                          & Analysis of the linguistic and the stylist characteristic of the ChatGPT and human feedback to detect patterns & Limited in the detection capability. The dataset is highly unbalanced.                                                                                                                                                                                         & Dataset                             & Claimed                                   \\ \hline
Bleumink et al.                     & Designed a web-based detection tool to detect texts in the education field                                     & Performed experiments only on the education data. Didn't specify the patterns found in the dataset analysis                                                                                                                                                 & Online Tool                         & Claimed                                   \\ \hline
Tang et al.                         & Analyzed the white-box and black-box detection techniques                                                      & Just a survey                                                                                                                                                                                                                                               & with (out) dataset                  & Claimed                                   \\ \hline
Mitchell et al.                     & AI-generated text detection using log probabilities computed by a generative model                             & Limited in the number of token that it can analyze                                                                                                                                                                                                          & Online Tool                         & Claimed                                   \\ \hline
Khalil et al.                       & Evaluation of plagiarism detectors on AI-generated essays                                                       & Only the analysis was conducted by the authors. Not an actual tool was designed. Focused only on the academic field.                                                                                                                                        & -                                   & Claimed                                   \\ \hline
Gao et al.                          & Evaluation of plagiarism detectors on AI-generated abstract                                                     & Very focused on academic abstracts. Using the existing detection tools for analysis.                                                                                                                                                                        &                                     & No                                        \\ \hline
Cotton et al.                       & AI-generated text detection using ChatGPT itself                                                               & ChatGPT is prone to claim that it has generated a text, even when this is not true.                                                                                                                                                                         & -                                   & Claimed                                   \\ \hline
Mitrović et al.                     & AI-generated text detection based on fine-tuned DistilBERT                                                      & Only studied the pros and cons of plagiarism effect of ChatGPT in the academic field.                                                                                                                                                                       &                                     & Claimed                                   \\ \hline
Ma et al.                           & AI-generated text detection based on "writing style"                                                           & It is difficult to automatically detect factual inconsistencies in the generated text.                                                                                                                                                                       &                                     & Claimed                                   \\ \hline
Kumarage et al.                     & Stylometric Detection of AI-generated text                                                                     & Sequence-based detection, require both human and AI-generated text.                                                                                                                                                                                         & GitHub                              & No                                        \\ \hline
Aharoni et al.                      & AI translated text detection                                                                                   & Only focus is text translation.                                                                                                                                                                                                                             & -                                   & No                                        \\ \hline
Kushnareva et al.                   & Topological Data Analysis for AI-generated text detection                                                      & Need white box access to the attention maps of the model generating text.                                                                                                                                                                                   & GitHub                              & No                                        \\ \hline
Gehrmann et al.                     & Support tool for manual AI-generated text detection                                                            & The detection is only visual, and the detection has to be made manually. The tool needs tuning and customization for each specific task. & Online Tool                         & Manual detection                          \\ \hline
Nguyen-Son et al.                   & Novel method for AI-generated text detection                                                                   & The effectiveness varies with the length of text in input. Tested only on text produced by a particular version of Google Translate.         & -                                   & No                                        \\ \hline
Zellers et al.                      & Fake news creation and detection                                                                                 & Do not consider adversarial robustness. The only focus is fake news.                                                                        & Online Tool                         & No                                        \\ \hline
Fröhling et al.                     & Classifier for AI-generated text detection                                                                     & The detection  becomes more difficult with increasing model complexity                                                                                                                                                                                      & -                                   & Claimed                                  
\end{tabular}

==> table/comparison_survey_horizontal.tex <==
\begin{tabular}{ccccc}
\textbf{Author(s)} & \textbf{Design, aims}                                                                                                                                           & \textbf{Limitations}                                                                                                                                                                      & \textbf{Available} & \textbf{Tested on GPT-3} \\ \hline
Solaiman et al.    & \begin{tabular}[c]{@{}c@{}}Analysis of the human detection,\\ automated ML-based detection of \\ synthetic texts using 3 models\end{tabular}                    & \begin{tabular}[c]{@{}c@{}}Limited in the detection capability. \\ Able to detect only the text \\ generated by ChatGPT-2\end{tabular}                                                    & Online Tool        & No                       \\ \hline
Guo et al.         & \begin{tabular}[c]{@{}c@{}}Analysis of the linguistic and \\ the stylist characteristic of\\  the ChatGPT and human feedback to \\ detect patterns\end{tabular} & \begin{tabular}[c]{@{}c@{}}Limited in the detection capability. \\ The dataset is highly unbalanced.\end{tabular}                                                                         & Dataset            & Claimed                  \\ \hline
Bleumink et al.    & \begin{tabular}[c]{@{}c@{}}Designed a web-based detection tool to \\ detect texts in the education field\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}Performed experiments only on the education data. \\ Di not specify the patterns found in the dataset analysis\end{tabular}                                    & Online Tool        & Claimed                  \\ \hline
Tang et al.        & \begin{tabular}[c]{@{}c@{}}Analyzed the white-box and \\ black-box detection techniques\end{tabular}                                                            & Just a survey                                                                                                                                                                             & with (out) dataset & Claimed                  \\ \hline
Mitchell et al.    & \begin{tabular}[c]{@{}c@{}}AI-generated text detection \\ using log probabilities computed by \\ a generative model\end{tabular}                                & Limited in the number of token that it can analyze                                                                                                                                        & Online Tool        & Claimed                  \\ \hline
Khalil et al.      & \begin{tabular}[c]{@{}c@{}}Evaluation of plagiarism detectors on\\ AI-generated essays\end{tabular}                                                             & \begin{tabular}[c]{@{}c@{}}Only the analysis was conducted by the authors. \\ Not an actual tool was designed. \\ Focused only on the academic field.\end{tabular}                        & -                  & Claimed                  \\ \hline
Gao et al.         & \begin{tabular}[c]{@{}c@{}}Evaluation of plagiarism detectors on \\ AI-generated abstract\end{tabular}                                                          & \begin{tabular}[c]{@{}c@{}}Very focused on academic abstracts. \\ Using the existing detection tools for analysis.\end{tabular}                                                           &                    & No                       \\ \hline
Cotton et al.      & \begin{tabular}[c]{@{}c@{}}AI-generated text detection \\ using ChatGPT itself\end{tabular}                                                                     & \begin{tabular}[c]{@{}c@{}}ChatGPT is prone to claim that \\ the text was generated by it, \\ even when this is not true.\end{tabular}                                                    & -                  & Claimed                  \\ \hline
Mitrović et al.    & \begin{tabular}[c]{@{}c@{}}AI-generated text detection based on \\ fine-tuned DistilBERT\end{tabular}                                                           & \begin{tabular}[c]{@{}c@{}}Only studied the pros and cons of \\ plagiarism effect of ChatGPT in\\ the academic field.\end{tabular}                                                        &                    & Claimed                  \\ \hline
Ma et al.          & \begin{tabular}[c]{@{}c@{}}AI-generated text detection based on \\ "writing style"\end{tabular}                                                                 & \begin{tabular}[c]{@{}c@{}}It is difficult to automatically detect \\ factual inconsistencies in \\ the generated text.\end{tabular}                                                      &                    & Claimed                  \\ \hline
Kumarage et al.    & \begin{tabular}[c]{@{}c@{}}Stylometric Detection of \\ AI-generated text\end{tabular}                                                                           & \begin{tabular}[c]{@{}c@{}}Sequence-based detection, \\ require both human and AI-generated text.\end{tabular}                                                                            & GitHub             & No                       \\ \hline
Aharoni et al.     & AI translated text detection                                                                                                                                    & Only focus is text translation.                                                                                                                                                           & -                  & No                       \\ \hline
Kushnareva et al.  & \begin{tabular}[c]{@{}c@{}}Topological Data Analysis for \\ AI-generated text detection\end{tabular}                                                            & \begin{tabular}[c]{@{}c@{}}Need white box access to \\ the attention maps of \\ the model generating text.\end{tabular}                                                                   & GitHub             & No                       \\ \hline
Gehrmann et al.    & \begin{tabular}[c]{@{}c@{}}Support tool for manual \\ AI-generated text detection\end{tabular}                                                                  & \begin{tabular}[c]{@{}c@{}}The detection is only visual, \\ and the detection has to be made manually. \\ The tool needs tuning and customization for \\ each specific task.\end{tabular} & Online Tool        & Manual detection         \\ \hline
Nguyen-Son et al.  & \begin{tabular}[c]{@{}c@{}}Novel method for \\ AI-generated text detection\end{tabular}                                                                         & \begin{tabular}[c]{@{}c@{}}The effectiveness varies with \\ the length of text in input. \\ Tested only on text produced by \\ a particular version of Google Translate.\end{tabular}     & -                  & No                       \\ \hline
Zellers et al.     & Fake news creation and detection                                                                                                                                & \begin{tabular}[c]{@{}c@{}}Do not consider adversarial robustness. \\ The only focus is fake news.\end{tabular}                                                                           & Online Tool        & No                       \\ \hline
Fröhling et al.    & \begin{tabular}[c]{@{}c@{}}Feature classifier for \\ AI-generated text detection\end{tabular}                                                                   & \begin{tabular}[c]{@{}c@{}}The detection  becomes more difficult with \\ increasing model complexity\end{tabular}                                                                         & -                  & Claimed                 
\end{tabular}

==> table/evaluation.tex <==
\begin{tabular}{|l|c|c|}
\hline
\textbf{Paper}         & \textbf{TPR(\%)} & \textbf{TNR(\%)} \\ \hline
Stylometric Detection of AI-generated text~\cite{kumarage2023stylometric}  & 13.3         & 84.7         \\ \hline
AICheatCheck~\cite{bleumink2023keeping}           & 21.8         & 92.5         \\ \hline
Topological artificial Text Detection~\cite{kushnareva2021artificial} & 34.1         & 86.3         \\ \hline
Grover~\cite{zellers2019defending}                 & 23.1         & 91.3         \\ \hline
Feature classifier for AI-generated text detection~\cite{Frohling2021feature}     & 33.8         & 89.2         \\ \hline
GLTR~\cite{gehrmann2019gltr}                  & 21.9         & 97.2         \\ \hline
ZeroGPT~\cite{AITextDetector}              & 32.5         & 92.3         \\ \hline
OpenAI Text Classifier~\cite{AITextClassifier}     & 27.9         & 91.8         \\ \hline
OpenAI GPT-2 Output Detector Demo~\cite{solaiman2019release}  & 7.4          & 97.8         \\ \hline
DetectGPT~\cite{mitchell2023detectgpt}              & 14.9         & 96.4         \\ \hline
GPTZero~\cite{GPTZero}                & 8.3          & 85.1         \\ \hline
Hugging Face~\cite{Huggingface}          & 9.1          & 96.9         \\ \hline
Content at Scale~\cite{aicontentdetector}      & 28.5         & 85.7         \\ \hline
Writer AI Content Detector~\cite{WriterAIContentDetector}     & 1.4          & 98.8         \\ \hline
Hello-SimpleAI~\cite{guo2023close}         & 44.6         & 98.6         \\ \hline
Corrector App~\cite{correctorapp}          &  0.9            & 98.8           \\ \hline
Writefull GPT Detector~\cite{writefull}          & 1.8          & 98.6         \\ \hline
Copyleaks~\cite{copyleaks}              & 1.5          & 98.7         \\ \hline
Draft and Goal~\cite{DAG}         & 1.7          & 98.7         \\ \hline
\end{tabular}

==> table/old_approach.tex <==
\begin{tabular}{|l|ll|l|l|ll|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Approach}} & \multicolumn{2}{c|}{Target Model}     & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Publicly \\ Available\end{tabular}}} & \multicolumn{1}{c|}{\multirow{2}{*}{Free/Paid}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}ChatGPT \\ Detection\end{tabular}} \\ \cline{2-3} \cline{6-7} 
\multicolumn{1}{|c|}{}                          & \multicolumn{1}{l|}{ChatGPT} & Others & \multicolumn{1}{c|}{}                                                                               & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{TPR}                      & \multicolumn{1}{c|}{TNR}                     \\ \hline
                                                & \multicolumn{1}{l|}{}        &        &                                                                                                     &                                                 & \multicolumn{1}{l|}{}                         &                                              \\ \hline
                                                & \multicolumn{1}{l|}{}        &        &                                                                                                     &                                                 & \multicolumn{1}{l|}{}                         &                                              \\ \hline
                                                & \multicolumn{1}{l|}{}        &        &                                                                                                     &                                                 & \multicolumn{1}{l|}{}                         &                                              \\ \hline
                                                & \multicolumn{1}{l|}{}        &        &                                                                                                     &                                                 & \multicolumn{1}{l|}{}                         &                                              \\ \hline
                                                & \multicolumn{1}{l|}{}        &        &                                                                                                     &                                                 & \multicolumn{1}{l|}{}                         &                                              \\ \hline
                                                & \multicolumn{1}{l|}{}        &        &                                                                                                     &                                                 & \multicolumn{1}{l|}{}                         &                                              \\ \hline
                                                & \multicolumn{1}{l|}{}        &        &                                                                                                     &                                                 & \multicolumn{1}{l|}{}                         &                                              \\ \hline
                                                & \multicolumn{1}{l|}{}        &        &                                                                                                     &                                                 & \multicolumn{1}{l|}{}                         &                                              \\ \hline
\end{tabular}

==> table/survey_justified.tex <==
\renewcommand\tabularxcolumn[1]{m{#1}}
\begin{tabularx}{\textwidth}{|l|X|X|c|c|c|}
\hline
\textbf{Paper}    & \textbf{Approach}                                                                                              & \textbf{Limitations}                                                                                                                    & \textbf{Available} & \textbf{Dataset} & \textbf{Verified} \\ \hline

Cotton et al. \cite{cotton2023ensuring} & AI-generated text detection using ChatGPT itself  & ChatGPT is prone to claim that the text was generated by it, even when this is not true              & -                    & -                & \textbf{$\times$}                  \\ \hline

Kumarage et al. \cite{kumarage2023stylometric} & Stylometric Detection of AI-generated text & Sequence-based detection, require both human and AI-generated text                                   & \checkmark           & -                & check                   \\ \hline

Ma et al. \cite{ma2023abstract} & AI-generated text detection based on the "writing style"  & It is difficult to automatically detect factual inconsistencies in the generated text                & -                    & -                & $N. A.$                    \\ \hline

Khalil et al. \cite{khalil2023will} & Evaluation of plagiarism detectors on AI-generated essays  & The authors conducted only the analysis. Not an actual tool was designed. Focused only on the academic field    & -    & -                & $N. A.$                     \\ \hline

Mitrović et al. \cite{mitrovic2023chatgpt} & AI-generated text detection based on fine-tuned DistilBERT                                                     & Only studied the pros and cons of plagiarism effect of ChatGPT in the academic field                                                    & -                    & -              & $N. A.$                  \\ \hline 

Mitchell et al. \cite{mitchell2023detectgpt} & AI-generated text detection using log probabilities computed by a generative model                             & Limited in the number of token that it can analyze                                                                                      & \checkmark         & -                & check                  \\ \hline

Guo et al. \cite{guo2023close} & Analysis of the linguistic and the stylist characteristic of the ChatGPT and human feedback to detect patterns & Limited in the detection capability. The dataset is highly unbalanced and comprises anomalous text instances                                                                   & \checkmark                    & \checkmark         & check                  \\ \hline

Bleumink et al. \cite{bleumink2023keeping} & Designed a web-based detection tool to detect texts in the education field                                     & Performed experiments only on the education data. Does not specify the patterns found in the dataset analysis                           & \checkmark         & -                & check                 \\ \hline

Gao et al. \cite{gao2022comparing} & Evaluation of plagiarism detectors on AI-generated abstract                                                    & Very focused on academic abstracts. Using the existing detection tools for analysis                                                     & -                     & -                 & \textbf{$\times$}                       \\ \hline

Kushnareva et al. \cite{kushnareva2021artificial} & Topological Data Analysis for AI-generated text detection                                                      & Need white box access to the attention maps of the model generating text                                                                & \checkmark              & -                & check                   \\ \hline

Fröhling et al. \cite{Frohling2021feature} & Feature classifier for AI-generated text detection                                                             & The detection  becomes more difficult with increasing model complexity                                                                  & \checkmark                     & \checkmark                 & check                \\ \hline

Zellers et al. \cite{zellers2019defending} & Fake news creation and detection                                                                               & Do not consider adversarial robustness. The only focus is fake news                                                                     & \checkmark         & -                & check                      \\ \hline

Solaiman et al. \cite{solaiman2019release} & Analysis of the human detection, automated ML-based detection of synthetic texts using 3 models                & Limited in the detection capability. Able to detect only the text generated by ChatGPT-2                                                & \checkmark         & -                & check                       \\ \hline

Gehrmann et al. \cite{gehrmann2019gltr} & Support tool for manual AI-generated text detection                                                            & The detection is only visual, and the detection has to be made manually. The tool needs tuning and customization for each specific task & \checkmark         & -                & \textbf{$\times$}         \\ \hline

Nguyen-Son et al. \cite{nguyen2017identifying} & Detection of AI-generated text using   & The effectiveness varies with the length of text in input. Tested only on text produced by a particular version of Google Translate     & -             & -                & \textbf{$\times$}        \\ \hline

Aharoni et al. \cite{aharoni2014automatic} & Detection of AI-translated text using automatic text classification methods with common content-independent linguistic features  & Main focus is only on text translation     & -                    & -                & $N. A.$                       \\ \hline
\end{tabularx}

==> table/survey_updated.tex <==
\begin{tabular}{llllll}
\textbf{Paper}    & \textbf{Approach}                                                                                              & \textbf{Limitations}                                                                                                                    & \textbf{Online Tool} & \textbf{Dataset} & \textbf{Tested on GPT-3} \\ \hline
Solaiman et al.   & \parbox{\linewidth}{Analysis of the human detection, automated ML-based detection of synthetic texts using 3 models}                & \parbox{\linewidth}{Limited in the detection capability. Able to detect only the text generated by ChatGPT-2}                                                & Online Tool          & -                & No                       \\ \hline
Guo et al.        & \parbox{\linewidth}{Analysis of the linguistic and the stylist characteristic of the ChatGPT and human feedback to detect patterns} & \parbox{\linewidth}{Limited in the detection capability. The dataset is highly unbalanced}                                                                   & -                    & Dataset          & Claimed                  \\ \hline
Bleumink et al.   & \parbox{\linewidth}{Designed a web-based detection tool to detect texts in the education field}                                     & \parbox{\linewidth}{Performed experiments only on the education data. Does not specify the patterns found in the dataset analysis}                        & Online Tool          & -                & Claimed                  \\ \hline
Mitchell et al.   & \parbox{\linewidth}{AI-generated text detection using log probabilities computed by a generative model}                             & \parbox{\linewidth}{Limited in the number of token that it can analyze}                                                                                      & Online Tool          & -                & Claimed                  \\ \hline
Khalil et al.     & \parbox{\linewidth}{Evaluation of plagiarism detectors on AI-generated essays}                                                      & \parbox{\linewidth}{The authors conducted only the analysis. Not an actual tool was designed. Focused only on the academic field}                            & -                    & -                & Claimed                  \\ \hline
Gao et al.        & \parbox{\linewidth}{Evaluation of plagiarism detectors on AI-generated abstract}                                                    & \parbox{\linewidth}{Very focused on academic abstracts. Using the existing detection tools for analysis}                                                     &                      &                  & No                       \\ \hline
Cotton et al.     & \parbox{\linewidth}{AI-generated text detection using ChatGPT itself}                                                               & \parbox{\linewidth}{ChatGPT is prone to claim that the text was generated by it, even when this is not true}                                                 & -                    & -                & Claimed                  \\ \hline
Mitrović et al.   & \parbox{\linewidth}{AI-generated text detection based on fine-tuned DistilBERT}                                                     & \parbox{\linewidth}{Only studied the pros and cons of plagiarism effect of ChatGPT in the academic field}                                                    &                      &                  & Claimed                  \\ \hline
Ma et al.         & \parbox{\linewidth}{AI-generated text detection based on the "writing style"}                                                       & \parbox{\linewidth}{It is difficult to automatically detect factual inconsistencies in the generated text}                                                   &                      &                  & Claimed                  \\ \hline
Kumarage et al.   & \parbox{\linewidth}{Stylometric Detection of AI-generated text}                                                                     & \parbox{\linewidth}{Sequence-based detection, require both human and AI-generated text}                                                                      & GitHub               & -                & No                       \\ \hline
Aharoni et al.    & \parbox{\linewidth}{AI translated text detection}                                                                                   & \parbox{\linewidth}{Only focus is text translation}                                                                                                          & -                    & -                & No                       \\ \hline
Kushnareva et al. & \parbox{\linewidth}{Topological Data Analysis for AI-generated text detection}                                                      & \parbox{\linewidth}{Need white box access to the attention maps of the model generating text}                                                                & GitHub               & -                & No                       \\ \hline
Gehrmann et al.   & \parbox{\linewidth}{Support tool for manual AI-generated text detection}                                                            & \parbox{\linewidth}{The detection is only visual, and the detection has to be made manually. The tool needs tuning and customization for each specific task} & Online Tool          & -                & Manual detection         \\ \hline
Nguyen-Son et al. & \parbox{\linewidth}{Novel method for AI-generated text detection}                                                                   & \parbox{\linewidth}{The effectiveness varies with the length of text in input. Tested only on text produced by a particular version of Google Translate}     & -                    & -                & No                       \\ \hline
Zellers et al.    & \parbox{\linewidth}{Fake news creation and detection}                                                                               & \parbox{\linewidth}{Do not consider adversarial robustness. The only focus is fake news}                                                                     & Online Tool          & -                & No                       \\ \hline
Fröhling et al.   & \parbox{\linewidth}{Feature classifier for AI-generated text detection}                                                             & \parbox{\linewidth}{The detection  becomes more difficult with increasing model complexity}                                                                  & -                    & -                & Claimed                 
\end{tabular}

==> testing_copy.tex <==
\section{Evaluation}
\label{sec:test_copy}

\noindent This section evaluates publicly available literature, tools, or codes that can differentiate between AI-generated and human-generated responses. \textit{Our primary focus is on the tools claiming to detect ChatGPT-generated content}. However, we also evaluate (to the best of our abilities) the performance of other AI-generated text detection tools that do not make explicit claims about detecting ChatGPT-generated content on ChatGPT prompts. To assess the effectiveness of these tools, we employ a benchmark dataset (Section \ref{sub:dataset}) that comprises prompts from ChatGPT and humans. Then, we measure the detection capabilities of these tools on both ChatGPT-generated and human-generated content and present the results in Table~\ref{tab:summary}.




\subsection{Benchmark Dataset}
\label{sub:dataset}
\noindent We utilized the inquiry prompts proposed by Guo et al.~\cite{guo2023close} through the OpenAI API\footnote{\url{https://openai.com/blog/introducing-chatgpt-and-whisper-apis}} to generate a benchmark dataset. This dataset comprises 58,546 responses generated by humans and 72,966 responses generated by the ChatGPT model, resulting in 131,512 unique samples that address 24,322 distinct questions from various fields, including medicine, open-domain, and finance. Furthermore, the dataset incorporates responses from popular social networking platforms, which provide a wide range of user-generated perspectives. To assess the similarity between human-generated and ChatGPT-generated responses, we employed the sentence transformer \mbox{\textit{all-MiniLM-L6-v2}}\footnote{\url{https://huggingface.co/sentence-transformers/all-MiniLM-L6-v2}}. Then, we selected responses with the highest and lowest levels of similarity to assemble a benchmark dataset, which was reduced to approximately 10\% of the primary dataset that we generated. This benchmark dataset serves as a standardized reference for evaluating the ability of different techniques to detect ChatGPT-generated content.


\subsection{Evaluation Metrics} 
\noindent To measure and compare the effectiveness of each approach, we utilized the following metrics:
\begin{itemize}
\item \textit{True Positive Rate (TPR): } This metric represents the tool's sensitivity in detecting text that ChatGPT generates. True Positive ($TP$) is the total number of correctly identified samples, while we consider False Negative ($FN$) the number of samples not classified as generated text or incorrectly identified as human text. Therefore, $TPR = \frac{TP}{TP+FN}$.
\item \textit{True Negative Rate (TNR):} This metric indicates the tool's specificity in detecting human-generated texts. True Negatives ($TN$) is the total number of correctly identified samples, while False Positives ($FP$) is the number of samples incorrectly classified as being produced by ChatGPT. Therefore, $TNR = \frac{TN}{TN+FP}$.
\end{itemize}


\subsection{Evaluated Tools and Algorithms} 
\noindent [Note: For the tools in the literature, Section \ref{sec:analysis} delineates their functionality. However, we provide a brief functionality for the tools available online in this section.] We evaluated several tools and algorithms, each with its unique functionality, as follows:

\begin{itemize}

\item \textit{Stylometric Detection of AI-generated Text}~\cite{kumarage2023stylometric}:
This tool utilizes stylometric signals to examine the writing style of a text by identifying patterns and features that are unique to them. These signals are then extracted from the input text to enable sequence-based detection of AI-generated tweets.

\item \textit{AICheatCheck}~\cite{bleumink2023keeping}:
A web-based tool that can detect whether a human or \textit{ChatGPT} generated a text. 

\item \textit{ZeroGPT}~\cite{AITextDetector}:
This tool is specifically developed to detect OpenAI text but has limited capabilities with shorter text.

\item \textit{OpenAI Text Classifier}~\cite{AITextClassifier}:
This fine-tuned GPT model developed by OpenAI predicts the likelihood of a text being AI-generated from various sources, including \textit{ChatGPT}. However, the tool only works with 1000 characters or more and is less reliable in determining if a text was artificially generated.

\item \textit{DetectGPT}~\cite{mitchell2023detectgpt}:
This tool only works with 48 tokens or more.

\item \textit{GPTZero}~\cite{GPTZero}:
This classification model determines whether a document was written by an LLM, providing predictions at a sentence, paragraph, and document level. However, it mainly works for content in the English language and only allows text with a character count between 250 and 5000 characters.

\item \textit{Hugging Face}~\cite{Huggingface}: 
This tool was released by Hugging Face for detecting text generated by \textit{ChatGPT}. However, it tends to over-classify text as being \textit{ChatGPT}-written.

\item \textit{Hello-SimpleAI}~\cite{guo2023close}:
This tool is designed explicitly for \textit{ChatGPT} and has undergone extensive human evaluations and linguistic analyses of ChatGPT-generated content compared to that of humans. However, the available dataset is highly unbalanced and comprises anomalous text instances.
The tool can identify only text with 2500 characters or less.

\item \textit{Perplexity (PPL})~\cite{perplexityAnalysis}: 
The perplexity (PPL) is a widely employed metric for assessing the efficacy of Large language models (LLM). It is calculated as the exponential of the negative average log-likelihood of text under the LLM. A lower PPL value implies that the language model is more confident in its predictions. LLMs are trained on vast text corpora, enabling them to learn common language patterns and text structures. Consequently, PPL can be utilized to gauge how effectively a given text conforms to such typical characteristics. 
%In their study, Guo et al.~\cite{guo2023close} employed the open-source GPT-2 small\footnote{\url{https://huggingface.co/gpt2}} model to compute PPL and reported that content generated by \textit{ChatGPT} exhibits relatively lower PPLs when compared to human-written text.

\item \textit{Writefull GPT Detector}~\cite{writefull}: 
It is primarily used for detecting plagiarism, this tool can identify if a piece of text is generated by \textit{GPT-3} or \textit{ChatGPT}. The tool consistently classified AI-generated texts with a probability score no higher than ~40\%.

\item \textit{Copyleaks}~\cite{copyleaks}: 
This tool claims to detect if a text is generated by \textit{GPT-3}, \textit{ChatGPT}, humans, or a combination of humans and AI. The tool accepts only text with 150 or more characters.

\item \textit{Chatting and cheating}~\cite{cotton2023chatting}: 
This tool uses \textit{ChatGPT} for AI-generated text detection. The chatbot is prone to claim that the text was generated by itself, inferring that the input text is likely to belong to its large training dataset.

\item \textit{Plagiarism Detection}~\cite{khalil2023will}: 
This study evaluates plagiarism detection tools on academic essays generated by \textit{ChatGPT}. The authors also asked \textit{ChatGPT} whether it generated the essay in question.

\item\textit{ChatGPT or human? Detect and explain}~\cite{mitrovic2023chatgpt}: 
This study uses a framework based on \textit{DistilBERT}, a lightweight model trained using \textit{BERT}, to detect \textit{ChatGPT}-generated two-line restaurant reviews. The model was fine-tuned using a Transformer-based approach. However, no tool or code is available for this study.

\item \textit{Content at Scale}~\cite{aicontentdetector}:
This is an online tool available to detect text generated by \textit{ChatGPT}. However, the tool can only analyze samples with 25000 characters or less.

\item \textit{Originality.ai}~\cite{originality}: 
This paid tool is designed to work with \textit{GPT-3}, \textit{GPT 3.5} (DaVinci-003), and \textit{ChatGPT} models. However, the tool only works with 100 words or more and is prone to classify \textit{ChatGPT}-generated content as real. %the site claim GPT 3.5 and ChatGPT, don't know if they mean GPT-3.5 or some other LLM

\item \textit{Writer AI Content Detector}~\cite{WriterAIContentDetector}: 
This tool is designed to work with \textit{GPT-3} and \textit{ChatGPT} models. However, its limitation restricts the amount of text that can be checked on each experiment to a maximum of 1500 characters.

\item \textit{Draft and Goal}~\cite{DAG}: 
This tool is intended for detecting content generated by \textit{GPT-3} and \textit{ChatGPT} models, and it is equipped to perform detection in both English and French. However, it has a requirement that the input text should be at least 600 characters or longer to work effectively.

\item \textit{Scientific abstracts comparison}~\cite{gao2022comparing}: 
This study compares \textit{ChatGPT}-generated academic paper abstracts using a plagiarism checker, a \textit{GPT-2} Output Detector, and human review. The plagiarism checker used in this study was RoBERTa.

\item \textit{Feature classifier for AI-generated text detection}~\cite{Frohling2021feature}
This algorithm uses feature-based detection to identify automated language models such as \textit{GPT-2}, \textit{GPT-3}, and \textit{Grover}. The detection becomes less accurate with increasing text complexity.

\item \textit{Topological Artificial Text Detection}~\cite{kushnareva2021artificial}:
This tool utilizes Topological Data Analysis to detect AI-generated text. However, it requires white box access to the attention maps of the model used for generating the text. The available code uses \textit{BERT} attention maps, and the authors claim that the tool is robust against unseen prompts from \textit{GPT-2} models.

\item \textit{OpenAI GPT-2 Output Detector Demo}~\cite{solaiman2019release}:
This tool was specifically developed by OpenAI to detect text generated by GPT-2.

\item \textit{GLTR}~\cite{gehrmann2019gltr}:
This tool utilizes the distributional properties of the underlying text used for the model and was tested on prompts from the GPT-2 1.5B parameter model. However, it only allows for visual classification, making it a manual human detection tool. Additionally, it requires tuning and customization for each specific task.

\item \textit{Grover}~\cite{zellers2019defending}:
This is a state-of-the-art defense against neural fake news, with a specific focus on detecting fake news. However, no research was conducted on GPT models, and it does not consider adversarial robustness~\cite{Frohling2021feature}.
\end{itemize}

